The T2K Side Muon Range Detector

The T2K experiment is a long baseline neutrino oscillation experiment aiming to observe the appearance of {\nu} e in a {\nu}{\mu} beam. The {\nu}{\mu} beam is produced at the Japan Proton Accelerator Research Complex (J-PARC), observed with the 295 km distant Super- Kamiokande Detector and monitored by a suite of near detectors at 280m from the proton target. The near detectors include a magnetized off-axis detector (ND280) which measures the un-oscillated neutrino flux and neutrino cross sections. The present paper describes the outermost component of ND280 which is a side muon range detector (SMRD) composed of scintillation counters with embedded wavelength shifting fibers and Multi-Pixel Photon Counter read-out. The components, performance and response of the SMRD are presented.

==> SMRD_elec.tex <==
% TRIP-t Electronics

The SMRD is using the same electronics as some of the other T2K near detectors 
P0D, ECAL and the INGRID) to read out the MPPCs. This electronics is based on the
TRIP-t ASIC\footnote{ASIC: Application Specific Integrated Circuit}
developed at Fermilab\cite{tript}. Signal from 64 MPPCs are routed to
custom designed front end boards (TFB)\footnote{The TFB (TRIP-t
  front-end board) was developed by Imperial College London.} that house
4 TRIP-t ASICs using miniature coax cables.  The signals from the
photosensors are capacitively split 1:10 and both routed to separate
channels of the ASIC to increase the dynamic range of the electronics.
A one photo-electron signal corresponds to around 10 ADC counts in the 
high gain channel, while the full scale signal in the low gain channel 
corresponds to 500 pe.

The TRIP-t chip is integrating the charge in programable integration
windows, which are synchronised with the neutrino beam structure. There
is a programmable dead time after each integration cycle, which is at
least 50 nsec long. The chip can store the result of 23 integration
cycles in a capacitor array. Once the 23 integration cycle have been
recorded, the data is multiplexed onto two dual channel 12-bit ADCs,
which digitise the data. Signal from the high gain
channel are routed to a discriminator, which is part of the TRIP-t
ASIC. The front-end board is controlled by an FPGA, which also
timestamps the output of the discriminator with a 2.5 sec
resolution. The threshold is programmable from 0 to 5 p.e.
The ADC and timestamp data is assembled by the FPGA and
send to a backend board for data concentration and buffering. The
output of the discriminators are also used to calculate trigger
primitives, which are used to initiate the readout of the detector for
cosmic ray muons. One normally requires hits from both ends of a scintillator 
panel and at least 2 panels to be hit, before a trigger primitive is transmitted 
to the cosmic trigger module.
Monitoring information (mainly temperature and
voltages) are also recorded by the TFB and asynchrony transmitted
to the RMM. More detail of the front end part of the electronics can
be found in \cite{TFB}.

The backend of the electronics system consists of a readout merger
modules (RMMs), cosmic trigger module (CTMs), several slave clock
modules (SCM) and a master clock module (MCM). All the boards have
been developed at the Rutherford Appleton Laboratory using a common
hardware platform, which has been build around a high end Vertex II
Pro FPGA from Xilinx, which is clocked at 100 MHz. 
The board can drive 14 high speed optical links
via its RocketIO and up to 192 LVDS links.

The signals from 32 TFBs, which are on the detector and around 3 m away 
from the photosensors, are routed to RMM via cat5e
cables. The RMM controls the TFBs, distributes the clock and trigger
signals and receives the data after a trigger signal was received by
the TFBs. It asynchrony sends this data via an Gigabit Ethernet
link to a commercial PC that collects and process the data. The RMM is
equipped with 500 MByte DDR2 memory and can buffer up to 128 triggers.
The RMM receives trigger and timing signals from the SCM (see below).

The master clock module receives signals from the accelerator that
determine when the neutrino spill happens and also from a GPS based
clock. The later signals are used to synchronise the electronics to
UTC. The MCM is also connected to the cosmic trigger modules, which
receive signals from up to 192 TFBs. All 128 TFBs used to read out 
the SMRD are used to generate the cosmic trigger. Readout is initiated,
if at least 2 TFBs on two different sides of the detector are generating
a trigger primitive in a 200 nsec window.
 All timing and trigger signals are
transmitted via the RocketIO driven optical link to the slave clock
modules. 

Bibliography

[tript]
"Bench Test of First TRIP-t Prototypes"
Leo Bellantoni, Paul Rubinov 
D0 note 4845

or 

J. Estrada, C. Garcia, B. Hoenison, and P. Rubinov, ÒMCM II and the
Trip chip,Ó D0 note 4009, Fermilab-TM-2226, Dec 2003.

[tfb]
"The front end readout system for the T2K-ND280 detectors"
Vacheret, A.;   Greenwood, S.;   Noy, M.;   Raymond, M.;   Weber, A.; 
Nuclear Science Symposium Conference Record, 2007. NSS '07. IEEE
Issue Date: Oct. 26 2007-Nov. 3 2007
On page(s): 1984 - 1991 


==> endcap.tex <==
\subsection{}

Write text here ...






==> geometry.tex <==
\subsection{}

Write text here ...





